Topological simplicity, commensurator super-rigidity and non-linearities of Kac-Moody groups

We provide new arguments to see topological Kac-Moody groups as generalized semisimple groups over local fields: they are products of topologically simple groups and their Iwahori subgroups are the normalizers of the pro-p Sylow subgroups. We use a dynamical characterization of parabolic subgroups to prove that some countable Kac-Moody groups with Fuchsian buildings are not linear. We show for this that the linearity of a countable Kac-Moody group implies the existence of a closed embedding of the corresponding topological group in a non-Archimedean simple Lie group, thanks to a commensurator super-rigidity theorem proved in the Appendix by P. Bonvin.

==> ResumeIF590.tex <==
\magnification=1150
\overfullrule=0pt
\parindent=0pt
\nopagenumbers 

\input amssym.def
\input amssym.tex

\def\pec{\vskip2mmplus1mmminus1mm}
\def\gec{\vskip4mmplus1mmminus1mm}

\def\og{\leavevmode\raise.3ex\hbox{$\scriptscriptstyle\langle\!\langle\,$}}
\def\fg{\leavevmode\raise.3ex\hbox{$\scriptscriptstyle\,\rangle\!\rangle\ $}}
\def\trait{\hbox{--- }}
\def\qed{\nobreak\hfill $\square$}
\def\page#1{\leaders\hbox to 5mm{.}\hfill \rlap{\hbox to 2mm{\hfill #1}}\par}

{\bf Pr\'epublication Institut Fourier 590 : } 

\pec 

Bertrand R\'EMY : 
{\it  Topological simplicity, commensurator super-rigidity and non-linearities of Kac-Moody groups}. 

\pec 

Appendix by Patrick BONVIN : {\it Strong boundaries and  commensurator super-rigidity}. 

\gec 

R\'esum\'e : 
Nous donnons de nouveaux arguments pour voir les groupes de Kac-Moody topologiques comme des
g\'en\'eralisations de groupes semi-simples sur des corps locaux : ils sont produits directs de groupes
topologiquement simples et leurs sous-groupes d'Iwahori sont les normalisateurs de leur pro-$p$ sous-groupes
maximaux. 
Nous utilisons une caract\'erisation dynamique des sous-groupes paraboliques pour montrer que certains
groupes de Kac-Moody de type fini \`a immeubles fuchsiens ne sont pas lin\'eaires. 
Nous montrons pour cela que la lin\'earit\'e d'un groupe de Kac-Moody de type fini implique l'existence d'un
plongement du groupe topologique correspondant dans un groupe de Lie simple non archim\'edien. 
Nous utilisons un th\'eor\`eme de super-rigidit\'e du commensurateur prouv\'e en appendice par P. Bonvin. 

\pec 

Mots-cl\'es : groupe de Kac-Moody, 
syst\`eme de Tits raffin\'e, 
groupe pro-$p$, 
r\'eseau, 
groupe de Lie simple non archim\'edien,
super-rigidit\'e du commensurateur, 
non lin\'earit\'e, 
immeuble de Bruhat-Tits, 
immeuble hyperbolique. 

\pec 

Classification AMS : 
22F50,
% Groups as automorphisms of other structures
22E20,
% General properties and structure of other Lie groups
51E24,
% Buildings and the geometry of diagrams
53C24,
% Rigidity results
22E40,
% Discrete subgroups of Lie groups
17B67.
% Kac-Moody algebras (structure and representation theory)

\gec 

\end


